Bayesian Nonparametric Erlang Mixture Modeling for Survival Analysis

We develop a flexible Erlang mixture model for survival analysis. The model for the survival density is built from a structured mixture of Erlang densities, mixing on the integer shape parameter with a common scale parameter. The mixture weights are constructed through increments of a distribution function on the positive real line, which is assigned a Dirichlet process prior. The model has a relatively simple structure, balancing flexibility with efficient posterior computation. Moreover, it implies a mixture representation for the hazard function that involves time-dependent mixture weights, thus offering a general approach to hazard estimation. We extend the model to handle survival responses corresponding to multiple experimental groups, using a dependent Dirichlet process prior for the group-specific distributions that define the mixture weights. Model properties, prior specification, and posterior simulation are discussed, and the methodology is illustrated with synthetic and real data examples.

==> old_files/01abs.tex <==
\begin{abstract}
In this article, we propose a Bayesian nonparametric model for Survival analysis. The model is built from structured mixture of Erlang densities mixing on shape parameters with a common scale parameter. The mixture weights are constructed through the increments of a distribution function which has a Dirichlet process (DP) prior. We further extend the model for the data arise from multiple groups with a common-weight dependent Dirichlet process (DDP) prior. The model enables the efficient posterior simulation by using Markov chain Monte Carlo (MCMC) algorithm and provides inferences with general functionals, such as density, survival, and hazard function. Synthetic and real data examples are provided for the illustration of the model. 
\end{abstract}
{\bf Keywords:} Survival Analysis; Dirichlet process; Erlang mixtures; Markov chain Monte Carlo; Right censoring



==> old_files/02intro.tex <==
\section{Introduction}

% In Survival analysis, researchers are interested in time-to-event data, such as, death of a person, discharge of a patient from hospital, or failure of a machine. Let $T$ be a random variable on the positive real line, $\mathbb{R}^+$, denoting the time to the event of interest. 
% The survival function of $T$ describes the probability surviving beyond time point $t$, $S(t) = Pr(T > t) = 1 - F(t)$, where $F(t)$ is the distribution function of $T$. The hazard function describes the instantaneous rate of occurrence of the event, $h(t)=lim_{\Delta t\to t}Pr(t<T\le t+\Delta t|T>t)/(\Delta t)=f(t)/S(t)$, where $f(t)$ is the density function of $T$. The cumulative hazard is a related quantity, defined by, $H(t)=\int_{0}^th(u)du$, which is also related to the survival function, $S(t)=exp(-H(t))$. The traditional methods for handling the survival data are described by \cite{klein1997}. Here, we focus on the Bayesian nonparametric approaches. 

Estimating different functionals with censored data has been an important topic in survival analysis. It is very common in clinical trials that survival times of a portion of subjects are not observed due to loss of track. Survival models must take both survival times and censored times into consideration.

Many models have been proposed in the literature, here, we focus on the Bayesian nonparametric (BNP) approaches. See \cite{Ibrahim_2001}, and \cite{Mueller_2015} chapter 6 for reviews of Bayesian survival analysis. 

Typical BNP methods construct priors for a specific functional on the space of random functions. Some early work focused on the point estimation of distribution function $F$. Such as, in \cite{SusarlaRyzin1976}, a DP prior is placed on the distribution function $F$, and \cite{FergusonPhadia1979} extended the work to the neutral to the right processes \citep{Doksum1974}. 
%The full inference of posterior distribution of $F$ was obtained by the development of simulation-based model fitting approaches. 
Later, the development of simulation-based model fitting approaches enable the full inference for posterior distribution of $F$. Such models include the mixture of DP (MDP) \citep{Antoniak1974} in \cite{Doss1994} and \cite{DossHuffer2003}, the mixture of P\'{o}lya trees \citep{Lavine1992} in \cite{MuliereWalker1997}, the DP mixture (DPM) model with a Weibull kernel in \cite{Kottas2006}, and the beta-Stacy process in \cite{WalkerMuliere1997}. 

Instead of placing priors on the distribution functions, the cumulative hazard and hazard functions can also be the target. In the context of modeling cumulative hazard function, there are Gamma process \citep{Kalbfleisch1978}, beta process \citep{Hjort1990}, and Bernstein polynomials \citep{Chang2005}. For hazard function estimation, \cite{DykstraLaud1981} developed the extended Gamma process.

In this paper, we propose a structured Bayesian nonparametric model for density estimation. The model is composed of mixture of Erlang densities mixing on integer shape parameters with a common scale parameter. The mixture weights are constructed through increments of some distribution function on the positive real line, $\mathbb{R}^+$. We refer the model as Erlang mixtures model. One of the attractive properties of the model is that its distribution function can converge pointwise to any continuous distribution function on the positive real line with certain conditions. This model can be applied to different fields under frequentist and Bayesian framework, such as queueing system \citep{Tijms}, insurance loss \citep{LinLee2010} with the mixture weights estimated by an EM algorithm, and medical expenditures \citep{Venturini_Dominici_Parmigiani_2008} with mixture weights estimated by a parametric Bayesian method, renewal process inter-arrival distributions \citep{XiaoS2020}, and Poisson process intensities \citep{Kim2021}, where the mixture weights in the latter two cases are estimated under Bayesian nonparametric framework. There has not been any exploration of the model for survival data. 

Motivated by the flexibility, we placed a Dirichlet process (DP) prior (\citeauthor{Ferguson1973} \citeyear{Ferguson1973}; \citeauthor{Antoniak1974} \citeyear{Antoniak1974}) on the distribution function which defines the mixture weigths.
% the distribution function that constructs the mixture weights is modeled under Bayesian nonparametric framework with a Dirichlet process (DP) prior (\citeauthor{Ferguson1973} \citeyear{Ferguson1973}; \citeauthor{Antoniak1974} \citeyear{Antoniak1974}). 
The Erlang mixtures model is able to capture different shapes of the density functions suggested by the data and it enables efficient algorithm for posterior simulation. 
% At the same time, in clinical trials, survival data are usually collected from multiple experimental groups, such as control and treatment groups. 
We also extended the Erlang mixtures model for the data arise from multiple experimental groups. To allow the borrowing strength across groups, we used a common-p DDP prior \citep{MacEachern2000}. The model allows crossing hazard rates and survival functions, which the two popular methods, proportional hazards (PH) model and the accelerated failure time (AFT) model can't reach. We also develop an efficient Markov chain Monte Carlo (MCMC) algorithm to fit the model for the posterior simulation and model inferences.

The paper is organized as follows. Section 2 introduces the model that do not include different experimental groups. We also discuss the posterior simulation and model inferences. Section 3 shows two synthetic data examples with data from a bimodal density and data contains right censoring. In section 4 and 5, we extend the basic model to incorporate with treatment and control groups and illustrate the model with synthetic data examples. Section 6 contains the conclusion and discussion of the possible extensions. 

==> old_files/03noCovModel.tex <==
\section{Methodology for survival data in one group}
The model development and model properties of the Erlang mixture model are discussed in Section \ref{sec:model1}. The prior specification, posterior simulation and model inferences are discussed in Section \ref{sec:model1priorspec} and Section \ref{sec:model1MCMC} respectively.

\subsection{The model description}
\label{sec:model1}
A survival random variable $T$ is defined on the positive real line, $\mathbbm{R}^+$. The density function of the proposed model is a structured mixture of Erlang densities mixing on shape parameters with a common scale parameter. An Erlang distribution is a special gamma distribution with an integer shape parameter. The density function is written as, 
\begin{align*}
f(t|M,\theta,G) &= \sum_{m=1}^M \omega_m ga(t|m, \theta) = \sum_{m=1}^M \omega_m \frac{1}{(m-1)!\theta^m} t^{m-1}e^{-\frac{t}{\theta}},
\end{align*}
where $ga(\cdot|m, \theta)$ denotes the density of a gamma distribution with mean $m\theta$. The mixture weights, $\{\omega_m:m=1,\dots,M\}$, are defined through the increments of a random distribution function $G$, $\omega_m = G(m\theta) - G((m-1)\theta)$, for $m = 1, \dots, M-1$, and $\omega_M = 1 - G((M-1)\theta)$. The distribution function of the Erlang mixtures model converges to $G$ pointwise, as $M \to \infty$ and $\theta \to 0$ \citep{LinLee2010}.

We show that survival and hazard functions also have the mixture representation of Erlang survival and hazard functions. 
$$
S(t|M,\theta,G) = \sum_{m=1}^M \omega_m S_{ga}(t|m,\theta) \textit{ and } h(t|M,\theta,G) = \sum_{m=1}^M \omega_m^*(t) h_{ga}(t|m, \theta),
$$
where $S_{ga}(\cdot|m,\theta)$ and $h_{ga}(\cdot|m,\theta)$ denote the survival and hazard functions of a gamma random variable with parameters $m$ and $\theta$. The mixture weights in the survival function remain the same with the ones in the density function while the mixture weights in the hazard function depend on time. Each time-dependent mixture weight is written as $\omega_m^*(t) = \frac{ \omega_m S_{ga}(t|m, \theta) }{ \sum_{j=1}^M \omega_j S_{ga}(t|j,\theta) }$. Although the hazard function of each Erlang random variable is non-decreasing, the time-dependent mixture weights allow the flexible shape of the hazard function of the Erlang mixture model. 

% The common scale parameter $\theta$ controls the fineness of the discretization of the distribution function $G$. To increases the accuracy of the fit, $\theta$ needs to decrease, and the model requires a large number of Erlang densities, i.e. a large M is desired. Jointly, $\theta$ and $M$ define the effective support of the model, it will be discussed in depth in the following sections. 

We model the mixture weights $(\omega_1, \dots, \omega_M)$ under the BNP framework by assigning a DP prior to $G$, $G \sim DP(\alpha, G_0)$. $\alpha$ is the DP precision parameter, and $G_0$ is the baseline centering distribution function. The DP precision parameter $\alpha$ controls the variability of $G$. For any $t \in (0,\infty)$, $G(t) \sim Beta(\alpha G(t), \alpha (1 - G(t)))$, and $Var(G(t)) = \frac{G_0(t)(1 - G_0(t))}{1+\alpha}$. The larger value of $\alpha$ leads to the closer realization of $G$ to $G_0$. Any distribution on $\mathbb{R}^+$ can be a good candidate for $G_0$, however, considering the simplicity and practicality, we found that an exponential distribution works sufficiently well in practice. For a fixed $M$, the mixture weights have a Dirichlet prior distribution with parameters as the increments on $G$, $(\omega_1, \dots, \omega_M) \sim Dir(G(\theta), \dots, 1-G((M-1)\theta))$. 
% Let $G_0$ be a distribution function of exponential density with both mean and variance at $b$, $G_0(\phi|b)=1-exp\left(-\frac{\phi}{b}\right)$. 


\begin{figure}[t]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering 
        \includegraphics[width=\linewidth]{fig/prior/weigths_M_50_theta_0.5_b_5_alpha_1.png}
        \caption{$\alpha=1$}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering 
        \includegraphics[width=\linewidth]{fig/prior/weigths_M_50_theta_0.5_b_5_alpha_10.png}
        \caption{$\alpha=10$}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering 
        \includegraphics[width=\linewidth]{fig/prior/weigths_M_50_theta_0.5_b_5_alpha_100.png}
        \caption{$\alpha=100$}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering 
        \includegraphics[width=\linewidth]{fig/prior/density_M_50_theta_0.5_b_5_alpha_1.png}
        \caption{$\alpha=1$}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering 
        \includegraphics[width=\linewidth]{fig/prior/density_M_50_theta_0.5_b_5_alpha_10.png}
        \caption{$\alpha=10$}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering 
        \includegraphics[width=\linewidth]{fig/prior/density_M_50_theta_0.5_b_5_alpha_100.png}
        \caption{$\alpha=100$}
    \end{subfigure}
    \caption{Erlang mixture model prior simulation. The plot includes the mixture weights (top panels) and density functions of Erlang mixture model (bottom panels) with different values of DP precision parameter. In the bottom panels, the red dashed lines represent the density functions of baseline distribution $G_0$. From left to right, the DP precision parameter $\alpha$ are set to be 1, 10, and 100. In all cases, $M=50$, $\theta=0.5$, and $b=5$.}
    \label{Fig:DP_weights}
\end{figure}

Figure \ref{Fig:DP_weights} illustrates mixture weights and the corresponding density functions. The top panels show that the model generates fewer "nonzero" mixture weights, note that all mixture weights are theoretically nonzero, but they can be sufficiently small in practice. The bottom panels show that the corresponding density functions are less discrepant from the baseline density as $\alpha$ increases. 

==> old_files/04noCovPriorSpec.tex <==
\subsection{Prior specification}
\label{sec:model1priorspec}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/prior/multi_density_M_100_theta_0.5_b_5_alpha10.png}
        \caption{$(M, \theta) = (100, 0.5)$}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/prior/multi_density_M_50_theta_1_b_5_alpha10.png}
        \caption{$(M, \theta) = (50, 1)$}
    \end{subfigure}%
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/prior/multi_density_M_20_theta_0.2_b_5_alpha10.png}
        \caption{$(M, \theta) = (20, 0.2)$}
    \end{subfigure}
    \caption{Prior realizations of density function from the Erlang mixtures model. The plot shows realizations of density function with $(M, \theta) = (100, 0.5)$ (left panel), $(M, \theta) = (50, 1)$ (middle panel), and $(M, \theta) = (20, 0.2)$ (right panel). For all cases, $b=5$ and $\alpha = 10$. In each panel, there are 5 different realizations (solid lines) from the prior and the density of baseline distribution (the dashed red line) on the interval $(0, T_0)$, where $T_0$ is the 99th percentile of the $G_0$.}
    \label{Fig:priorspec_DP}
\end{figure}

Each Erlang density in the model has mean value equal to $m\theta$. The common scale parameter $\theta$ controls the fineness of the discretization of the distribution function $G$. As $\theta$ decreases, the accuracy of the fit increases, and the model requires a large number of Erlang densities. Thus $\theta$ and $M$ jointly define the effective support of the model. 

Figure \ref{Fig:priorspec_DP} shows the 5 prior realizations from the Erlang mixtures model for 3 different combinations of $(M, \theta)$, $(50,1)$, $(20, 0.2)$, and $(100, 0.5)$, for all cases $b=5$ and $\alpha=10$. 
The 99th percentile of the baseline distribution, $exp(5)$, is below the value of $M\theta$ in the left and middle panels, but beyond the one in the right panel. Therefore, $M\theta$ needs to be sufficiently large to provide enough effective support. 


To complete the Bayesian story, we place a gamma prior distribution on $\alpha$, and an inverse gamma prior distribution on $b$. In general, we suggest that the baseline centering distribution function should have a large effective support covering the largest observation or the potential largest observation. Conditional on $b$, the 99th percentile of $G_0$ equals $blog(100)$. We assign $b$ a prior distribution whose mean is greater than $t_{(n)}/log(100)$, where $t_{(n)}$ denotes the largest or the potential largest observation. It is equivalent to say the expectation of 99th percentile of $G_0$ is larger than $t_{(n)}$. 

We consider a joint prior distribution for $M$ and $\theta$ with a hierarchical form. Let $\theta$ have a marginal gamma prior distribution. If prior information suggests nonstandard and complex density function, the hyperparameters should form a gamma distribution that favors small values of $\theta$. Conditional on $\theta$, we place a discrete uniform distribution on $M$, $\left\{ \ceil{M_1/\theta}, \dots, \ceil{M_2/\theta} \right\}$, where $M_1$ and $M_2$ are pre-specified constants. We recommend that $M_1= max(2, \ceil{M^*})$ and $M_2 = cM_1$, where $M^*$ is the largest or the potential largest observed value, $\ceil{M^*}$ is the smallest integer that is larger or equal to $M^*$. $c$ is a constant and can be set at any integer between 2 and 10. A large $c$ is suggested when the potential observations are likely to be larger than the largest observed value. 
Since the baseline centering distribution has a determined shape, the prior of $\alpha$ is considered to favor small values so that the model has more flexibility learning from the data. 



==> old_files/05noCovMCMC.tex <==
\subsection{Posterior simulation}
\label{sec:model1MCMC}
In this section, we discuss the posterior computation. Survival data are often right censored, that is, events are only observed up to a time point before the failure. For $i$th subject, let $T_i$ be the survival time and $C_i$ be the right censoring time. The final recorded time is denoted by $Z_i = min(T_i, C_i)$. $\nu_i$ denotes the binary censoring indicator, $\nu_i=0$ if $z_i = c_i < t_i$, and $\nu_i=1$ if $z_i=t_i$. The likelihood function of all observations is a combination of density and survival functions, as,
$$
L(\theta,M,G;data) = \prod_{i=1}^n \left[f(z_i|\theta, M,G)\right]^{\nu_i} \left[S(z_i|\theta, M,G)\right]^{1-\nu_i}.
$$

Recall that the mixture weights $(\omega_1, \dots, \omega_M)$ follows a Dirichlet distribution and $M$ is assumed to be random. The dimension of the mixture weights changes along with $M$ in each iteration of posterior computation. It will cause inefficiency of the computation. The key to solve the problem is by introducing latent variables to identify the mixture component assignments for each observation. Let $(\phi_1, \dots, \phi_n)$ denote the latent variables, which are iid from $G$, the linkage between Erlang mixtures model and latent variables is given in the following representation, 
$$
\sum_{m=1}^M \omega_m Ga(t|m, \theta) = \int_0^\infty \sum_{m=1}^{M-1} \mathbbm{1}_{((m-1)\theta,m\theta]}(\phi)Ga(t|m,\theta) + \mathbbm{1}_{((M-1)\theta,\infty)}(\phi)Ga(t|M,\theta)dG(\phi).
$$ 

The new representation forms a DP mixture model, thus we can develop a Gibbs sampler based on the P\'{o}lya urn scheme \cite{blackwell1973}. Each latent variable $\phi_i$ arises after marginalizing $G$ over its DP prior (\citeauthor{EscobarWest1995} \citeyear{EscobarWest1995}; \citeauthor{Neal2000} \citeyear{Neal2000}). The full model inferences with different functionals are based on sampling from the posterior distribution of $G$ \citep{Gelfand2002}. The details of the posterior computation are described in the Appendix. The full conditional of latent variable $\phi_i$ after integrating over the random measure $G$ is
\begin{align*}
\phi_i |& \{ \phi_{i'}: i' \ne i\}, t_i, \alpha, b, \theta, M \sim \\
& \frac{\alpha q_0}{\alpha q_0 + \sum^{n^{*-}}_{j=1}n^-_jq_j} f^*(\phi_i|t_i, \theta, M, b) + \sum^{n^{*-}}_{j=1} \frac{n_j^- q_j}{\alpha q_0 + \sum_{k=1}^{n^{*-}} n^-_kq_k}\delta_{\phi_j^{*-}}(\phi_i),
\end{align*}
where $q_0=\sum_{m=1}^M\omega^0_m[ga(t_i|m,\theta)]^{\nu_i}[S_{ga}(t_i|m,\theta)]^{1-\nu_i}$, $\omega^0_m=G_0(m\theta)-G_0((m-1)\theta)$, for $m=1,\dots,M-1$, and $\omega^0_M=1 - G_0((M-1)\theta)$, $q_j=k(t_j|\phi_j^*,\theta,M)$, $\phi_j^{*-}$ is a set of distinct values in the set $\{ \phi_{i'}:i' \ne i\}$, and $f^*(\phi_i|t_i, \theta, M, b)$ is the posterior distribution of the $\phi_j$ with respect to kernel function $k(t_i|\phi_j, \theta, M)$. Specifically, $f^*(\phi_j|t_i,\theta, M)$ is a piecewise density composed by truncated densities of the baseline centering distribution function $G_0$ on different intervals. Here, $f^*(\phi_j|t_i, \theta, M) = \sum_{m=1}^M\Omega_mTexp_m(\phi_j|b,1)$. $Texp_m$ is a truncated exponential density  on the interval $((m-1)\theta, m\theta]$ and $\Omega_m$'s are the rescaling weights, as $\Omega_m=\omega^0_m[ga(t_i|m,\theta)]^{\nu_i}[S_{ga}(t_i|m,\theta)]^{1-\nu_i}/q_0$. 

Sampling $(\theta, M)$ requires the Metropolis Hasting algorithm since there is no closed form for their joint posterior distribution. If the prior distribution of $b$ is set as $invga(b_\alpha, b_\beta)$, by the conjugation, the posterior distribution of $b$ is still an inverse gamma distribution, $invga(b_\alpha+n^*, b_\beta+\sum_{j=1}^{n^*}\phi^*_j)$, where $(\phi_1^*, \dots, \phi_{n^*}^*)$ are the distinct $\phi_i$'s. We use data augmentation method \cite{EscobarWest1995} to sample from the posterior distribution of the DP precision parameter $\alpha$. 

==> old_files/06synthetic1.tex <==
\section{Data examples}
In this section, we show two synthetic data examples. Section \ref{sec:bimodal} contains the data generated from a bimodal density. Section \ref{sec:upsidedown} contains the data generated from a unimodal density with different percentages of right censorship. 

\subsection{Bimodal density}
\label{sec:bimodal}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/M_trace.png}
        \caption{M}
    \end{subfigure}%
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/theta_trace.png}
        \caption{$\theta$}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/alpha_trace.png}
        \caption{$\alpha$}
    \end{subfigure}%
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/b_trace.png}
        \caption{$b$}
    \end{subfigure}
    \caption{Synthetic data from a bimodal density. Trace plots of posterior samples for $M$ and $\theta$}
    \label{fig:trace_bimodal}
\end{figure}

\begin{figure}[t]
    \centering 
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/M_hist.png}
        \caption{M}
    \end{subfigure}%
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/theta_hist.png}
        \caption{$\theta$}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/alpha_hist.png}
        \caption{$\alpha$}
    \end{subfigure}%    
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/b_hist.png}
        \caption{b}
    \end{subfigure}
    \caption{Synthetic data from a bimodal density. Histograms of posterior samples for $M$ (blue histograms), $\theta$, $\alpha$, and $b$ (grey histograms) and their corresponding prior distributions for $M$ (red histograms), $\theta$, $\alpha$, and $b$ (red dashed lines).}
    \label{fig:pos_bimodal} 
\end{figure}


\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/density.png}
        \caption{Density}
    \end{subfigure}
         &  
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/survival.png}
        \caption{Survival}
    \end{subfigure}\qquad
         \\
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn1/hazard.png}
        \caption{Hazard}
    \end{subfigure}
         & 
    \end{tabular}
    \caption{Synthetic data from a bimodal density. (a), (b), and (c) show the point estimates (dashed red line), 95\% uncertainty bands (shaded area), and the truth (solid black line) for the density, survival, and hazard functions, respectively.}
    \label{fig:functionals_bimodal}
\end{figure}

In the first synthetic example, data are generated from a bimodal density with 300 survival time points. The distribution is a mixture of two log-normal distributions, $0.4LN(0, 0.4)+0.6LN(2, 0.2)$. We first place an exponential prior on $\alpha$ with mean 1 and an inverse gamma prior on $b$ with shape and scale parameters 3 and 4, respectively. Then let $\theta$ have an exponential prior with mean 1 and $M$ have a conditional prior distribution, in particular, a discrete uniform distribution, $Unif\left\{ \ceil*{\frac{13}{\theta}}, \dots, \ceil*{\frac{39}{\theta}} \right\} $. After burn in and thinning, we obtain 2000 posterior samples. The mixing and convergence are diagnosed graphically through the trace plots in Figure \ref{fig:trace_bimodal}. We show the prior and posterior plots in Figure \ref{fig:pos_bimodal}. In (a), (b), (d) the posterior histograms have obvious shifts from the prior distributions. The estimation of different functionals are displayed in Figure \ref{fig:functionals_bimodal}. The Erlang mixture model captures bimodaility of the density function. The uncertainty bands (red shaded areas) cover the true functions (black solid lines). 

==> old_files/07synthetic2.tex <==
\subsection{Unimodal density with censoring}
\label{sec:upsidedown}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn2/density.png}
        \caption{Density} 
    \end{subfigure}
         &
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn2/survival.png}
        \caption{Survival}
    \end{subfigure}
         \\
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn2/hazard.png}
        \caption{Hazard}
    \end{subfigure}
         & 
    \end{tabular}
    \caption{Synthetic data from a unimodal density. Histograms of posterior samples for $M$ (blue histograms), $\theta$, $\alpha$, and $b$ (grey histograms) and their corresponding prior distributions for $M$ (red histograms), $\theta$, $\alpha$, and $b$ (red dashed lines).}
    \label{fig:functionals_upsidedown}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn2C1/density.png}
        \caption{Density. 10-15\%}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn2C1/survival.png}
        \caption{Survival. 10-15\%}
    \end{subfigure}
    \\
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn2C2/density.png}
        \caption{Density. 20-25\%}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn2C2/survival.png}
        \caption{Survival. 20-25\%}
    \end{subfigure}
    \\
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn2C3/density.png}
        \caption{Density. 30-35\%}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn2C3/survival.png}
        \caption{Survival. 30-35\%}
    \end{subfigure}
    \end{tabular}
    \caption{Synthetic data from a unimodal density containing different percentages of censorship. The first row has data with 13.33\% censoring, the second row has 20.33\% censoring, and the third row has 30.67\% censoring. The left and right panels show the posterior mean estimate (dashed red line), the posterior 95\% interval estimates (shaded area), and the truth (solid black line) of density functions and survival functions respectively. The fully observed survival times are displayed as histograms in the left panels.}
    \label{fig:censoring_upsidedown}
\end{figure} 


In the second synthetic data example, the data are generated from a log-normal distribution, $LN(0,0.5)$, with 300 survival times. Similar to the first example, we place an exponential prior with mean 1 on $\alpha$ and an inverse gamma prior on $b$ with shape and scale parameters 3 and 1, respectively. And let $\theta$ have an exponential prior distribution with mean 1. Conditional on $\theta$, let M have a discrete uniform prior distribution, $Unif\left\{\ceil*{\frac{5}{\theta}}, \dots, \ceil*{\frac{15}{\theta}}\right\}$. In Figure \ref{fig:functionals_upsidedown}, (a), (b), and (c) show the density, survival, and hazard function estimates, respectively. The point estimates (red dashed lines) capture the shapes of different functionals with uncertainty bands (shaded areas) covering most true functions (black solid lines). 

Then, we add independent and random censoring to the data set with different percents of censorship, in particular, we set the percentages at 10-15\%, 20-25\% and 30-35\%. In Figure \ref{fig:censoring_upsidedown}, the estimated density and survival functions for each case are shown. The model works for all cases and the width of the uncertainty bands increases as the percentage of censored data increases. 


==> old_files/08realData1.tex <==
\subsection{Lung cancer data}
\label{sec:lung}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/lung/density.png}
        \caption{Density}
    \end{subfigure}
         &  
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/lung/survival.png}
        \caption{Survival}
    \end{subfigure}\qquad
         \\
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/lung/hazard.png}
        \caption{Hazard}
    \end{subfigure}
         & 
    \end{tabular}
    \caption{Lung caner data. (a), (b), and (c) show the point estimates (dashed red line), and 95\% uncertainty bands (shaded area) for the density, survival, and hazard functions, respectively.}
    \label{fig:functionals_lung}
\end{figure}

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|c|c|c}
        \hline \hline 
        Survival time & (days) & Status & (freq.) \\ \hline 
        Max &  1022 & Censored & 63 \\ 
        Median & 255.5 & Death & 165 \\ \hline \hline 
    \end{tabular}
    \caption{Summary of lung cancer data}
    \label{tab:lungCancer}
\end{table}

The real data example is involving a lung cancer clinical trial. The survival times of 228 patients with advanced lung cancer from North Central Cancer Treatment group \citep{Loprinzi1994}. The dataset also includes covariates such as age, gender, and weight loss in last six months of the experiment, but here we only consider the survival times and censoring status. The summary of data used in the paper is summarized in Table \ref{tab:lungCancer}.

Let $\alpha$ have an exponential prior distribution with mean 1 and $b$ have an inverse gamma prior distribution with shape and scale parameters 3 and 230 respectively. Let $\theta$ have a gamma prior distribution with mean and variance $50$ and let $M$ have a discrete uniform distribution, $Unif\left\{\ceil*{\frac{1100}{\theta}},\dots, \ceil*{\frac{5500}{\theta}}\right\}$. 

% The left panel in Figure \ref{fig:lung} shows the posterior point (mean) and interval (95\% credible interval) estimates of the survival function under Erlang mixture model. For  comparison, the right panel in the same plot shows the data as a Kaplan-Meier curve. The two plots have the similar shape, and due to censoring, the uncertainty bands in the left panel keeps wide at the tail. The estimate shows the Erlang mixture model has a good fit for the lung cancer data. 

Figure \ref{fig:functionals_lung}(a), (b), and (c) show the point estimates (red dashed lines) and 95\% uncertainty bands (red shaded areas) of density, survival and hazard functions, respectively. The Erlang mixture model suggests a unimodal density function and  a monotonically increasing hazard function. 

==> old_files/09covModel.tex <==
\section{Modeling for control-treatment studies}
In Section \ref{sec:model2}, we show the the model extension for control-treatment experimental groups. Synthetic and real data example are in Section \ref{sec:diffmod} and Section \ref{sec:smallcellslung}.

\subsection{The Erlang mixture model extension}
\label{sec:model2} 
Survival data may arise from multiple experimental groups, here we consider the simplest case, control-and-treatment studies. A model being able to describe the correlation between two groups is desired. Let $x \in \mathcal{X}=\{C, T\}$ be the state space, where $C$ and $T$ represent control and treatment groups, respectively. Let $\theta$, $M$ and $G$ be covariate-dependent. The Erlang mixture model is then extended to 
$$
f_x(t|\boldsymbol{M}, \boldsymbol{\theta}, G) = \sum_{m=1}^{M_x} \omega_m(x) ga(t|m, \theta_x),
$$
where $\boldsymbol{\theta} = (\theta_C, \theta_T)$, and $\boldsymbol{M}=(M_C, M_T)$. The mixture weights is defined through a covariate-dependent distribution function $G_x$, $\omega_m(x) = G_x(m\theta_x)-G_x((m-1)\theta_x)$, for $m = 1, \dots, M-1$, and $\omega_M(x) = 1 - G_x((M-1)\theta_x)$. The two extreme modeling approaches for  $G_{\mathcal{X}}$ are (i) assuming two independent distribution functions $G_C$ and $G_T$, or (ii) assuming two identical distribution functions $G=G_C=G_T$. Either approach may not be suitable for most cases, so a flexible modeling approach that allows moderate borrowing strength across groups is expected. Naturally, we chose to use a DDP prior \citep{MacEachern2000}. $G_x$ has an almost sure representation \citep{Sethuraman1994} and can be written as $G_x=\sum_{l=1}^{\infty} p_{lx} \delta_{\phi^*_{lx}}$, where both atoms and weights are covariate-dependent. 

Motivated by the computational efficiency, we consider a single-p DDP model where the weights are shared by different groups and defined as $p_1 = v_1$, $p_l = v_l\prod_{r=1}^{l-1} (1 - v_r)$ for $l \ge 2$, $v_r \iidsim Beta(1, \alpha)$ and the atoms $\boldsymbol{\phi}^*_l$ are identically and independently arised from a bivariate distribution, $G_{0}$. There is a rich literature on the single-p DDP, including but not limited to \cite{Iorio2004}, \cite{Gelfand2005}, \cite{Iorio2009}, and \cite{Fronczyk2014}. The dependence between groups is introduced through the correlation of atoms. 



==> old_files/10covPriorSpec.tex <==
% \subsection{Prior specification}
% \label{sec:model2priorspec}

Since the scale parameter $\theta$ controls the fineness of discretization of the distribution function $G$, using the same $\theta$ for both control group and treatment is too restrictive. It is likely to cause overfitting for one group and underfitting for the other one. We consider independent priors for each $\theta_x$. The same prior specification strategy is applied here. A gamma prior is placed on $\theta_x$ and a discrete uniform distribution is placed on $M_x$, as $M_x|\theta_x\sim Unif\left\{ \ceil*{ \frac{ M_{x1} }{\theta_x}}, \dots, \ceil*{\frac{M_{x2}}{\theta_x}} \right\}$, where $M_{x1}$ and $M_{x2}$ are pre-specified constants.

For the baseline centering distribution, we let $G_0$ be a bivariate lognormal distribution with parameters $\mu$ and $\Sigma$, where $\mu = (\mu_1,\mu_2)'$, $\Sigma = ( (\Sigma_{11}, \Sigma_{12})',$ $(\Sigma_{12}, \Sigma_{22})')$. One of the good properties of a bivariate lognormal distribution is that the conditional distributions and marginal distributions remain lognormal. The prior choice for the precision parameter $\alpha$ is the same. 


Let $\mu$ have a bivariate normal prior distribution, $\mu \sim N_2(\mu_0, \Sigma_0)$, where $E(\mu)=\mu_0$. Let $\Sigma$ have an inverse Wishart prior distribution, $\Sigma \sim InvWishart(c,C)$, where $E(\Sigma)= C/(c-3)$. Since $\mu$ and $\Sigma$ determine the shape of the bivariate baseline distribution $G_0$, we suggest to set $\mu_0$ to be empirical mean of data with a log transformation, and $\Sigma_0$ to be a diagonal matrix with relative large diagonal elements. For $\Sigma$, we suggest to consider values where the marginal expectation of 99th percentile of $G_{0C}$ and $G_{0T}$ over priors cover the largest observation in each group.



==> old_files/11covMCMC.tex <==
% \subsection{Posterior inference} 
% \label{sec:model2MCMC}
The same data augmentation method can be used here to avoid the change of the dimension of the parameter space.
\begin{align*}
f_x(t|\boldsymbol{M},\boldsymbol{\theta},G) =& \int k_x(t|\boldsymbol{M}, \boldsymbol{\theta}, \boldsymbol{\phi}) dG_x(\boldsymbol{\phi}) \\
k_x(t|\boldsymbol{M}, \boldsymbol{\theta}, \boldsymbol{\phi}) =& \sum_{m=1}^{M_x-1}\boldsymbol{1}_{((m-1) \theta_x,m\theta_x]}(\phi_x)ga(t|m,\theta_x) \\
&+ \boldsymbol{1}_{((M_x-1)\theta_x, \infty)}( \phi_x)ga(t|M_x, \theta_x),
\end{align*}
where $\boldsymbol{\phi}=(\phi_C, \phi_T)$. By marginalizing over the random distribution function $G$, we have the following expression,
$$
\boldsymbol{\phi_i} | \boldsymbol{\phi_{-i}}, \mu, \Sigma \sim \frac{\alpha}{\alpha + n - 1}G_0(\boldsymbol{\phi_i}|\mu,\Sigma) + \frac{1}{\alpha+n-1}\sum_{j\ne i}\delta_{\boldsymbol{\phi_j}}(\boldsymbol{\phi_i}),
$$
where $\boldsymbol{\phi_{-i}}=\{\boldsymbol{\phi_1}, \dots, \boldsymbol{\phi_{i-1}}, \boldsymbol{\phi_{i+1}}, \dots, \boldsymbol{\phi_n} \}$, the set of all latent variables excluding the ith one. And $\boldsymbol{\phi^{*-}}$ is the set of all distinct elements in $\boldsymbol{\phi_{-i}}$. For $i=1,\dots,n$, the posterior distribution is a mixture of $n^{*-}$ point masses and posterior distribution of $\boldsymbol{\phi_i}$ based on $t_i$,

\begin{align*}
\boldsymbol{\phi_i}|& \boldsymbol{\phi_{-i}}, \mu, \Sigma, t_i, x_i, \boldsymbol{\theta}, M \sim \\
 &\frac{\alpha q_0}{\alpha q_0 + \sum_{j=1}^{n^{*-}}n_j^-q_j} f^*(\boldsymbol{\phi_i}|\mu, \Sigma, t_i, x_i, \boldsymbol{\theta}, M) + \frac{1}{\alpha q_0 + \sum_{j=1}^{n^{*-}}n_j^- q_j} \sum_{j\ne i}\delta_{\boldsymbol{\phi^{*-}_j}}(\boldsymbol{\phi_i}),
\end{align*}
where $q_j$ is the kernel function for ith observation evaluated at $\phi_j^{*-}$. $f^*(\phi_i|t_i,\mu,\Sigma,x_i,\theta,M)$ is the posterior distribution of a kernel function based in ith observation. $q_0$ is a normalizing constant, $q_0 = \sum_{m=1}^M D_{x_im} Ga(t_i|m, \theta(x_i))$, where $D_{x_im} = G_{0x_i}(m\theta(x_i)) - G_{0x_i}((m-1)\theta(x_i))$, for $m=1,\dots,M$, and $D_{x_iM} = 1 - G_{0x_i}((M-1)\theta(x_i))$. The algorithm of drawing posterior samples from the above distribution is described in appendix. There is no closed form for the posterior distribution of $\theta$, we use Metropolis algorithm for its posterior sampling. There are closed form for the posterior distribution of $\mu$ and $\Sigma$. $\mu|- \sim N_2(\mu|\mu_1, \Sigma_1)$, where $\Sigma_1 = \left[\Sigma_0^{-1} + {n^*}\Sigma^{-1} \right]^{-1}$, $\mu_1 = \Sigma_1 \left[ \Sigma_0^{-1}\mu_0 + \Sigma^{-1} \sum_{i=1}^{n^*} log(\phi_i)\right]$. $\Sigma | - \sim InvWishart_2(\Sigma|c_1, C_1)$, where $c_1=c+{n^*}$, $C_1 = C+\sum_{i=1}^{n^*}[log(\phi_i)-\mu][log(\phi_i)-\mu]^T$. 

==> old_files/12synthetic4.tex <==
\section{Synthetic data example - two group cases}
\label{sec:diffmod}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/thetaC_trace.png}
        \caption{$\theta_C$}
    \end{subfigure}
        &
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/MC_trace.png}
        \caption{$M_C$}
    \end{subfigure}
        \qquad \\
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/thetaT_trace.png}
        \caption{$\theta_T$} 
    \end{subfigure}
        &
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/MT_trace.png}
        \caption{$M_T$}
    \end{subfigure}
    \end{tabular}
    \caption{(a), (b), (c) and (d) show the trace plots of $\theta_C$, $M_C$, $\theta_T$, and $M_T$, respectively.}
    \label{fig:diff_modality_trace}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/thetaC_hist.png}
        \caption{$\theta_C$}
    \end{subfigure}
    &
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/thetaT_hist.png}
        \caption{$\theta_T$}
    \end{subfigure}
    \qquad \\
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/mu_hist1.png}
        \caption{$\mu_1$}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/mu_hist2.png} 
        \caption{$\mu_2$}
    \end{subfigure} \qquad
    \\
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/Sigma_hist11.png}
        \caption{$\Sigma_{11}$}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{fig/syn3/Sigma_hist22.png} 
        \caption{$\Sigma_{22}$}
    \end{subfigure}
    \end{tabular}
    \caption{Posterior histograms of $\theta_C$, $theta_T$, $\mu_1$, $\mu_2$, $\Sigma_{11}$, and $\Sigma_{22}$, and their prior distributions (red solid line)}
    \label{fig:diff_modality_poshist}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn3/densityC.png}
        \caption{Density, control group}
    \end{subfigure} 
    &
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn3/densityT.png}
        \caption{Density, treatment group} 
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn3/joint_survival.png}
        \caption{Survival}
    \end{subfigure}
    &
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/syn3/joint_hazard.png}
        \caption{Hazard} 
    \end{subfigure}    
    \end{tabular}
    \caption{Synthetic data from two groups with different modality. (a) and (b) show the point estimates (red dashed line), 95\% uncertainty bands (red shaded area), and the truth (black solid line) of the density function for control and treatment groups, respectively. (c) and (d) show the survival and hazard estimates.}
    \label{fig:diff_modality}
\end{figure} 
In this synthetic data example, data are generated from two groups with different modalities. Control group: $LN(0.5, 0.6)$. Treatment group: $0.4LN(0, 0.4)$ + $0.6LN(2, 0.2)$. The priors are set as following, $\alpha \sim exp(1)$, $\mu \sim N((log(2.02), log(4.90))', 10^3I_2)$, where $I_2$ is a 2$\times$ 2 diagonal matrix, $\Sigma \sim inv\mhyphen Wishart(4,I_2)$, $\theta_x \indsim exp(1)$, $M_x \indsim Unif\left\{\frac{12}{\theta_x},\dots,\frac{48}{\theta_x}\right\}$. 

The posterior convergence and mixing can be checked in Figure \ref{fig:diff_modality_trace}. The posterior histograms in Figure \ref{fig:diff_modality_poshist} show the obvious shift from the priors (red solid lines), which indicates significant learning from the data. 

The functional estimates of density, survival, and hazard functions are shown in Figure \ref{fig:diff_modality}. (a) and (b) indicate that the Erlang mixture model can successfully capture the different modalities of density functions. The uncertainty bands cover the truth very well for different functions. 

==> old_files/13synthetic5.tex <==
\subsection{Different weights}
\label{sec:diffweights}

\begin{figure}[t]
\centering
\begin{tabular}{cc}
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/thetaC_trace.png}
    \caption{$\theta_C$, trace plot}
\end{subfigure}
&
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/thetaC_hist.png}
    \caption{$\theta_C$, histogram}
\end{subfigure}
\\
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/thetaT_trace.png}
    \caption{$\theta_T$, trace plot} 
\end{subfigure}
&
\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/thetaT_hist.png}
    \caption{$\theta_T$, histogram}
\end{subfigure}
\end{tabular}
\caption{(a) and (c) show the trace plots of $\theta_C$ and $\theta_T$ with 95\% credible interval (red solid line), and (b) and (d) show the posterior histogram of $\theta_C$ and $\theta_T$ with prior density (red dashed line)}
\label{fig:diff_weights_trace}
\end{figure}


\begin{figure}[t]
\centering
\begin{subfigure}{0.25\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/mu_hist1.png}
    \caption{$\mu_1$}
\end{subfigure}%
\begin{subfigure}{0.25\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/mu_hist2.png} 
    \caption{$\mu_2$}
\end{subfigure}%
\begin{subfigure}{0.25\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/Sigma_hist11.png}
    \caption{$\Sigma_{11}$}
\end{subfigure}%
\begin{subfigure}{0.25\textwidth}
    \includegraphics[width=\linewidth]{fig/diff_weights/Sigma_hist22.png} 
    \caption{$\Sigma_{22}$}
\end{subfigure}
\caption{Posterior histograms of $\mu_1$, $\mu_2$, $\Sigma_{11}$, and $\Sigma_{22}$, and their prior distributions (red solid line)}
\label{fig:diff_weights_poshist}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/diff_weights/densityC.png}
        \caption{Density function, control group}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/diff_weights/densityT.png}
        \caption{Density function, treatment group} 
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/diff_weights/joint_survival.png}
        \caption{Survival function}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/diff_weights/joint_hazard.png}
        \caption{Hazard function}
    \end{subfigure}    
    \caption{Synthetic data from model where both the control and treatment groups have bimodal densities but with different weights for each mode. The top left panel shows the density estimate for control group data, the plot contains the histogram of simulated data, the posterior mean estimate of density (dashed red line), the 95\% posterior interval estimates (shaded area), and the truth of density function (black solid line). Top right panel shows the same plot but for treatment group. The bottom left panel shows the posterior mean estimates of survival function of control group (red dashed line), 95\% posterior interval estimates (red shaded area), ground truth (red solid line), and estimates for treatment group are in blue. The bottom right panel shows the estimates of hazard functions for control group and treatment group.}
    \label{fig:diff_weights}
\end{figure}


This synthetic data example shows the Erlang mixture model can capture the shape the densities of data whose densities under control and treatments groups have a bimodal shape but different weights for each mode. The control group data is generated from $lognormal(0.5,0.6)$ and the treatment group data is generated from $0.4lognormal(0, 0.4)$ + $0.6lognormal(2, 0.2)$. The average of observations for control and treatment groups are 3.11 and 4.93 respectively. And the largest observations for each group are 14.11 and 13.12. Following the discussion of prior specification in the previous section, we set priors as $\alpha \sim exp(1)$, $\theta_C \sim exp(1)$, $\theta_T \sim exp(1)$, $\mu_0=(log(3.11), log(4.93))$, $\Sigma_0 = 10^3I_2$, where $I_2$ is a 2 $\by$ 2 diagonal matrix, and $c=4$ along with $C=I_2$ as we don't expect correlation between control and treatment groups. The trace plots and posterior histogram of $\theta_C$ and $\theta_T$ are in Figure \ref{fig:diff_weights_trace}, with fair mixing. The marginal posterior distribution for $\mu_1$, $\mu_2$, $\Sigma_{11}$, and $\Sigma_{22}$ are shown in Figure \ref{fig:diff_weights_poshist}. Figure \ref{fig:diff_weights} illustrates point and interval estimates for density functions for control and treatment groups separately, survival and hazard functions together. The Erlang mixture model captures the bimodality for both groups and is able to assign the correct corresponding weight for each mode. 

==> old_files/14realData2.tex <==
\subsection{Small cells lung cancer data}
\label{sec:smallcellslung}
\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
     \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/smallcells/densityC.png}
        \caption{Density, control group}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/smallcells/densityT.png}
        \caption{Density, treatment group}
    \end{subfigure} 
    \qquad \\
     \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/smallcells/joint_survival.png}
        \caption{Survival}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/smallcells/joint_hazard.png}
        \caption{Hazard}
    \end{subfigure}     
    \end{tabular} 
    \caption{    \label{fig:small_cells_lung} Small cells lung data. (a) and (b) show the point estimates (red dashed line), 95\% uncertainty bands (red shaded area), and the truth (black solid line) of the density function for control and treatment groups, respectively. (c) and (d) show the survival and hazard estimates.} 
\end{figure}

% 300, 600, 1000, 1500, 1900
\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/smallcells/diff_surv_1.png}
    \caption{$t=100$}
    \end{subfigure}        
         &  
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/smallcells/diff_surv_2.png}
    \caption{$t=300$}
    \end{subfigure}         
         \qquad \\
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/smallcells/diff_surv_3.png}
    \caption{$t=600$}
    \end{subfigure}
         & 
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/smallcells/diff_surv_4.png}
    \caption{$t=1000$}
    \end{subfigure}
    \qquad \\
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/smallcells/diff_surv_5.png}
    \caption{$t=1500$}
    \end{subfigure}
    &
    \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/smallcells/diff_surv_6.png}
    \caption{$t=1900$}
    \end{subfigure}
    \end{tabular}
    \caption{Small cell lung cancer data. Posterior histograms for the difference in survival functions between Arm A and Arm B, at 6 time points, $t=100,300,600,1000,1500,1900$ days. Between the verticals lines are the 95\% credible intervals.}
    \label{fig:small_lung_cell_surv_diff}
\end{figure}

\begin{table}[ht!]
    \centering
    \begin{tabular}{c|c|c|c}
        \hline \hline 
        Survival time & (days) & Status & (freq.) \\ \hline 
        Arm A (Max) & 1980 & Arm A (Censored) & 15\\  
        Arm A (Median) & 623 & Arm A (Death) & 47 \\ \hline  
        Arm B (Max) & 1820 & Arm B (Censored) & 8 \\ 
        Arm B (Median) & 395 & Arm B (Death) & 51 \\ \hline 
    \end{tabular}
    \caption{Summary of small cells lung cancer data}
    \label{tab:small_cell_lung_cancer}
\end{table}

We apply the Erlang mixture model to survival times of patients with small cells lung cancer data \cite{Ying1995}. The data have survival times of patients who were randomly assigned to one of two treatments, Arm A and Arm B. The summary of data is shown in Table \ref{tab:small_cell_lung_cancer}. This dataset has also been studied by \cite{Poynor2019} for mean residual life functions using Bayesian nonparametric methods. 

The priors are set to $\alpha \sim ga(1,1)$, $\theta_x \indsim ga(1, 50)$, $M_x \indsim Unif\left\{\ceil*{\frac{3000}{\theta_x}}, \dots, \ceil*{\frac{15000}{\theta_x}}\right\}$, $\mu \sim N_2((6.7, 6.3), 10I_2)$, and $\Sigma \sim InvWishart(4, 0.5I_2)$.

Figure \ref{fig:small_cells_lung} shows the point estimates and 95\% uncertainty bands for density, survival, and hazard functions using the Erlang mixture model. The Erlang mixture model suggests single modal densities for both Arm A and Arm B according to (a) and (b). In (c), the estimated survival function of patients in Arm A is above the one of patients in Arm B. (d) indicates the hazard function in both groups have a upside-down bathtub shape hazard functions. 

Figure \ref{fig:small_lung_cell_surv_diff} shows the gap between survival functions of two groups, $S_A(t) - S_B(t)$, at time $t=100,300, 600, 1000, 1500, 1900$. At time 100, 300, 600, and 1000 days, the difference between the two treatment is clear, the patients receiving Arm A have significant higher survival curve. The difference diminishes at 1500 days and 1900 days. 

==> old_files/15discussion.tex <==
\section{Discussion}

We have proposed a model under Bayesian nonparametric framework modeling functions of interest in survival analysis. The model is built from a mixture of Erlang densities which share the scale parameter. The mixture weights is defined through an increments of a distribution function $G$ which is modeled nonparametric using a DP prior. We have extended the basic model to control-treatment study, where the random measure $G$ is extended as $\{G_C,G_T\}$ and modeled using a DDP prior, and the model remains flexibility and computational feasibility. Synthetic data examples are provided. 
